On Using Time Without Clocks via Zigzag Causality

Even in the absence of clocks, time bounds on the duration of actions enable the use of time for distributed coordination. This paper initiates an investigation of coordination in such a setting. A new communication structure called a zigzag pattern is introduced, and shown to guarantee bounds on the relative timing of events in this clockless model. Indeed, zigzag patterns are shown to be necessary and sufficient for establishing that events occur in a manner that satisfies prescribed bounds. We capture when a process can know that an appropriate zigzag pattern exists, and use this to provide necessary and sufficient conditions for timed coordination of events using a full-information protocol in the clockless model.

==> nonFFIP.tex <==
% !TEX root = postpodc17.tex
%
\Cref{thm:vzz}, that was presented in \Cref{sec:using}, assumes that the protocol in use is an \ffip, where upon delivery of a message, an agent sends immediately messages on all of its outgoing channels.
Doesn't it apply for a non \ffip? The answer is no. The reason behind it is the methods in which information can be conveyed.
Recall that a $\sigma$-visible zigzag pattern contains Lamport's happened before relation from the head nodes of the zigzag's forks (all but the last one). 
This relation grants $\sigma$ the knowledge that each head node occurs before (or at the same time as) the tail node of the next fork. 
Using a protocol that is an \ffip, the only mean to convey (new) information is by a message chain.
In a protocol that is not an \ffip, the information can be passed in an alternative method.

More formally, using a protocol that is an \ffip, if $\sigma$ knows that some external message was delivered, there must be a (not necessarily direct) message chain from the node that received the external event, to $\sigma$ (can be proved by generalizing \Cref{lem:past}). 
Thus, we can say that the only mean to convey information about the occurrence of spontaneous events (external messages deliveries) is by a message chain.
Another option to convey such information, as appear in \cite{BzMacm,LamSM}, is achieved by avoiding from sending a message, which is also considered as sending a \emph{null message}.
For example, in a system with synchronized clocks and constant delay on messages transmission time, we can agree that I send you a message in each second, unless I'll get some specific phone call.
In this case, if you see that a second has passed and you didn't receive a new message from me, then you know that I received that phone call.
Clearly, this option is not relevant when using an \ffip, as an agent cannot decide at some point not to send a message.
If we take a protocol that is not an \ffip, can we use this concept, of conveying information by not sending messages, in our system?
Note that such scheme contains an agent that decides at a specific time point (due to a specific local state) to avoid from sending a message (although he could send a message), and another node of the agent to whom the message wasn't sent, that must recognize the fact that the source agent could, but did not send a message.
Clearly the problematic part is how the node of the destination agent can find out that indeed some message wasn't sent.

Let $\Rrep=\Rrep(\gamma,P)$, where $P$ is an FIP protocol (each message contain the local state of its sender), but not an \ffip.
Fix $r\in\Rrep$, and let $\sigma$ be an $i$-node in $r$ and $\sigma'$ be a $k$-node in $r$, such that $\sigma'\lamr\sigma$.
Clearly, if $\sigma'$ avoided from sending a message to $i$, then $\sigma$ recognizes it, as it ``sees'' $\sigma'$, and knows that in this local-state, agent~$k$ won't sent a message. Exactly for this reason, that $\sigma$ already ``sees'' $\sigma'$, this avoidance cannot convey any new information to $\sigma$.
Now, let $p$ be a path in $\Net$, and assume that $\tet=\nodeF{\sigma',p}$ is a $\sigma$-aware node that appears in $r$ and that $\sigma$ knows of its existence, and that $\tet\not\lamr\sigma$.
Why do we have to say that $\tet$ appears in~$r$, and that $\sigma$ knows of its existence? 
Because once the protocol is not an \ffip, not all the $\sigma$-aware nodes necessarily appear in~$r$ (except for those that are in $\past(r,\sigma)$), and even if they do appear, it might be not known by $\sigma$ (i.e., there is another equivalent run in which $\sigma$ is found, but those nodes don't).
Assume that~$\tet$ is a $j$-node, and that $(j,i)\in\Chan$.
As $\tet\not\lamr\sigma$, then clearly agent~$i$ didn't receive in~$r$ a message from $\basic(\tet,r)$ before time $\timeof_r(\sigma)$.
Now, we can ask if $\sigma$ knows that $\tet$ didn't send a message.
Note that while $\sigma$ probably doesn't know exactly the local state of $\tet$, it might know some parts of it, and that might be enough to conclude if $\tet$ sends the message or doesn't.
But, if $\sigma$ concludes that way that $\tet$ doesn't send a message to $i$, it once again doesn't convey any new information, because the conclusion of this fact came from knowing part of the past of $\tet$.
For $\tet$ to truly convey information to $\sigma$, it must be that the part of the past of $\tet$ that is known by $\sigma$, is not enough to conclude if $\tet$ sends a message or doesn't.
%In another words, this fact must be concluded from observing the communication pattern.

To make stuff more formal, our current question is this:
Fix $r\in\Rrep$, and let $\sigma$ be a basic node in~$r$.
Assume that $\sigma$ knows that some node received an external message $e\in\Ext$.
Moreover, assume that~$e$ is delivered in $r$ to $\sigma'$.
What can we tell about the communication pattern that exists in $r$?
Note that in an \ffip, it is simply required that $\sigma'\lamr\sigma$.
It is not necessarily the case, however, for a non \ffip.
\asaQ{Example... based on fig1.}

 Recall the extended bounds graph $\GE{r,\sigma}$. Clearly $\sigma$ can construct this graph also in a non \ffip\ (as long as the protocol is still an FIP).
 So, can we find some valid timing function on this graph, and construct a run?
 We might be able to do so, in which case we can prove that it must be that $\sigma'\lamr\sigma$ [by not letting the environment to deliver external messages to nodes not from $\past(r,\sigma)$].
 However, it might be that there is no valid timing function on $\GE{r,\sigma}$.
Recall that \GE{r,\sigma} is constructed under the assumption of an \ffip. 
 This means that it assumes that any message that goes outside $\past(r,\sigma)$, will cause a flooding (i.e., its receiving node will send messages on all of its out links, and so will do the nodes that will receive those messages and so on).
Thus, if we find a correct timing, it means that it is indeed possible to do such flooding (if the protocol wanted to).
 If we don't, it means that it is 100\%\ sure that there was no complete flooding, as such flooding would have cause some message not from the past of $\sigma$, to be received in its past (and so it won't be ``$\sigma$'' anymore).

The condition for when there is no valid timing, is the existence of a positive cycle in \GE{r,\sigma}.
We can see any positive cycle in \GE{r,\sigma} as concatenation of alternate non empty sequences of original nodes and auxiliary nodes, where the number of sequences of original nodes equals the number of sequences of  auxiliary nodes.
Assume that it contains a single sequence of auxiliary nodes (and so also a single sequence of original nodes). What does it means?
A sequence of auxiliary nodes together with an original node that comes after that sequence, defines a node.
Assume that $S=(\psi_{i_c}, \psi_{i_{c-1}},\ldots,\psi_{i_1})$ is the auxiliary nodes sequence, and $\sigma_{i_0}$ is the original node that comes after this sequence in the positive cycle. Define $q=[i_0,i_1,\ldots,i_c]$. Then $S$ (together with $\sigma_{i_0}$) defines the node $\nodeF{\sigma_{i_0},q}$.
If this node appears in $r$, it must come after the boundary node of $i_c$ (agent $i_c$'s last node that appears in the past of $\sigma$).
The weight of the path $\ocomp{S}{\sigma_{i_0}}$ in \GE{r,\sigma} is $-\ubSym(q)$. This corresponds to the inequality $\timeof_r(\sigma_{i_0})\geq\timeof_r(\nodeF{\sigma_{i_0},q})+(-\ubSym(q))$.
Assume that $\sigma_{i_c}$ is the boundary node of $i_c$, and note that it must be the original node that comes before $S$ in the positive cycle (as the only way to go from an original node to an auxiliary node is by walking from the boundary node).
As the cycle is positive, it means that there is a path $P$ in \GE{r,\sigma} (only between original nodes, according to our assumption) from $\sigma_{i_0}$ to $\sigma_{i_c}$, such that $\weight(P)\geq\ubSym(q)$. As any path in \GE{r,\sigma} that contains only original nodes is also a path in \GB{r}, then $\timeof_r(\sigma_{i_c})\geq\timeof_r(\sigma_{i_0})+\ubSym(q)$. 
Combining the two inequalities, we get that $\timeof_r(\sigma_{i_c})\geq\timeof_r(\nodeF{\sigma_{i_0},q})$ which is impossible, as we know that $\timeof_r(\sigma_{i_c})<\timeof_r(\nodeF{\sigma_{i_0},q})$, if indeed \nodeF{\sigma_{i_0},q} appears in~$r$.
Thus, we get that \nodeF{\sigma_{i_0},q} simply doesn't appear in~$r$.
This means that there is some proper prefix of $q$, say $q'$, such that $\tet'=\nodeF{\sigma_{i_0},q'}$ appears in $r$, but that it doesn't send message to the agent that follow $q'$ in $q$. 
We name $\basic(\tet',r)$ as the \defemph{cut node}.
Note that $\sigma$ may not know who was the cut node.
Yet, this node can truly pass information to $\sigma$. % (even though $\sigma$ don't know who have passed that information).
For example, assume that the protocol forces all nodes to send messages, unless they received the external message $e$, and assume that $\basic(\tet',r)$ receives it.
And so, $\sigma$ recognizes that there was a message chain that wasn't sent, and it knows that it must be because some node along this message chain has received $e$.

And what about a (simple) cycle with two sequences of auxiliary nodes?
It defines two message chains, that it cannot be that both appear in $r$.
Note, however, that each of them might indeed appear, but not both together.
%If one of these message chains indeed appears, then observing the last node in the other chain that still appears in~$r$, i.e. the ``cut node'', then it might have passed us information.
%But, what if both don't fully appear in $r$? 
%[If we don't force that there will be no two identical external messages delivered in a single run, then no problem. But this might cause problems with earlier definitions... otherwise we are getting a bit out of optimality, as it might be that in such case no information can be passed (as long as there is no way in which both nodes can conclude the occurrence of the spoken event, without the observer concludes it... On the other hand, if we assume an observer that reads from the messages only the communication data, then it might not conclude the occurrence of the event. But, it will be still required from the other nodes to be able to conclude it both] 
More generally, any simple positive cycle forces that at least one of the messages chains that are represented by the auxiliary nodes sequences (and the basic nodes that comes just after then), cannot appear in any run $r'\in\Rrep$ where $r'\sim_\sigma r$.

Our next goal is to define a generalization for \Cref{thm:vzz} that also applies to non \ffip s.
First, we extend the notion of $\GE{r,\sigma}$ to $\GE{r,V}$ where $V$ is a set of basic nodes that appear in $r$. $\GE{r,V}$ is constructed based on the basic bounds graph (\GB{r}) that is induced by $V$, with the extension of the auxiliary nodes and the other edges as described in the definition of $\GE{r,\sigma}$, where every time we have used ``$\past(r,\sigma)$'' we should use ``$V$'' instead.  Thus, for example, $\GE{r,\sigma}=\GE{r,\past(r,\sigma)}$.

We start by defining $V=past(r,\sigma)$, $G=\GE{r,V}$
We find all the cut nodes in $r$ w.r.t G, add them and all the basic nodes in their pasts to $V$, and reconstruct $V$.
The idea is that allegedly any of the newly introduced node can convey information to $\sigma$.
We repeat the above stages, i.e. finding the cut nodes, and adding them and the nodes in their pasts to $V$, until there are no more cut nodes.
Note that convergence is promised, as the nodes that can be cut nodes (at any iteration) are only those whose time in $r$ is earlier than $\timeof_r(\sigma)$.
We define the \defemph{extended past} of $\sigma$, $\Vex_\sigma=V$, to be the set of nodes that appear in $V$ at the point of convergence, and say that $\sigma''\lamext\sigma$ iff $\sigma''\in \Vex_\sigma$.
At this point, we can truly find a valid timing function, that will produce us a valid run.
Then, in a similar manner to the proof of \Cref{thm:vzz}, we can prove that the existence of a $\sigma$-visible zigzag, where every instance of Lamport's happened before relation that was required is replaced with an instance of ``$\lamext$'', is a necessary condition for the knowledge at $\sigma$ concerning time difference between two nodes.


% A TEST, WHICH ACTUALLY TELLS NOTHING:
%More formally, we define the \emph{parasitic protocol test}:
%Note that we can define the protocol of agent $j$, to have a specific action for $\tet$.
%I.e., if in some run~$r$ agent $j$ receives a message chain along $p$ from $\sigma'$, then it performs the respective action.
%And so we change the protocol of $j$ so that $\tet$ will send a message either if it do so according to the original protocol, or if it receive an external message.
%Now, if under the new protocol it is assured that $\tet$ didn't send a message to $\sigma$, then $\tet$ has passed the test, and it might convey information to $\sigma$.
%Otherwise...  unfortunately it still might convey information to $\sigma$.
%This is because there is a case where $\sigma$ knows that at least one of two (or more) nodes, say $\tet$ and $\tet'$, didn't send a message, but it cannot tell for sure which one. In this case, all those nodes together convey information.
%\asaQ{It is generally problematic, as we said that only \tet\ follows that ``parasitic protocol''. }

% DEFINITION OF A TEST COMPLETELY WITHOUT A PROTOCOL:
%Observe $\sigma$, its past, and all of the $\sigma$-aware nodes that $\sigma$ knows that are exists ($\tet$ amongst them).
%Now assume that you don't know the protocol that created that run.
%Can you tell in this case, that $\tet$ didn't send a message to $\sigma$?
%If yes, then $\tet$ has passed the test, and so it might convey information. 
% If not... unfortunately it doesn't mean anything yet (both due to the case of ``one of many'', or that there is more protocol-dependent timing information).
 
 % OTHER GARBAGE:
%In such case, the only way that $\sigma$ can conclude that $\tet$ doesn't send a message, is only by recognizing that $\timeof_{r'}(\sigma)-\timeof_{r'}(\tet)>\upb{ji}$ holds for each run $r'$ such that $r'\sim_\sigma r$, i.e. that $(\Rrep,r)\models\Ksub{\sigma}(\tet\atleast{\upb{ji}+1}\sigma)$. \asaQ{How can we prove this? For that cause we need to somehow formalize the previous statement. Note that the last case is true even when we don't know the current protocol. Maybe this is the point?}
%
%
%We 
%have already seen that~$\sigma$ can obtain this knowledge, based on 
%%already know how can $\sigma$ has such knowledge, using 
%a $\sigma$-visible zigzag with weight of more than $\upb{ji}$.\footnote{One must be careful here, as it must be known by $\sigma$ that all the nodes that appear in the zigzag pattern are in fact exist in $r$.}
%In such case, $\tet$ might have conveyed $\sigma$ some information.
%For example, assume that $\tet$ avoids of sending such a message only if it receives a particular external message~$\mu$. Then $\sigma$ knows that~$\mu$ has been delivered.  %the relevant external message was delivered.
%It also might convey information about the past of $\tet$.
%%
%%Recall that in the $\sigma$-visible zigzag, the head nodes of the forks (except for the last fork) are in the past of $\sigma$, so that there is a message chain from them to $\sigma$, and this is what gives $\sigma$, among others, the knowledge on the concatenation of the forks.
%%Now, a null message can do just the same. I.e., $\tet$ can avoid sending a message only if it didn't see the tail node of some fork, and so it be used to build a visible zigzag.
%%There is here some kind of recursion, as we identify that $\tet$ avoided from sending a message using a visible zigzag, and then $\tet$ can be used to construct another visible zigzag, which can be used to conclude that another node didn't send a message
%
%
%
%%However, there is an importance nuance in a protocol that is not an FFIP.
%%While in an FFIP protocol, the sending pattern of messages is globally known (for example, if I send some agent a message, I know exactly to whom he will send messages when he will receive my message). In a non FFIP protocol, it might be non trivial question. For example, if I send some agent a message, this agent's protocol might be to send messages upon receiving my message, only if he receive some specific message from another agent before that. As I possibly cannot tell if he indeed received such message, I don't know what he shall do.



